Polynomial-Time Computation of Optimal Correlated Equilibria in Two-Player Extensive-Form Games with Public Chance Moves and Beyond

Unlike normal-form games, where correlated equilibria have been studied for more than 45 years, extensive-form correlation is still generally not well understood. Part of the reason for this gap is that the sequential nature of extensive-form games allows for a richness of behaviors and incentives that are not possible in normal-form settings. This richness translates to a significantly different complexity landscape surrounding extensive-form correlated equilibria. As of today, it is known that finding an optimal extensive-form correlated equilibrium (EFCE), extensive-form coarse correlated equilibrium (EFCCE), or normal-form coarse correlated equilibrium (NFCCE) in a two-player extensive-form game is computationally tractable when the game does not include chance moves, and intractable when the game involves chance moves. In this paper we significantly refine this complexity threshold by showing that, in two-player games, an optimal correlated equilibrium can be computed in polynomial time, provided that a certain condition is satisfied. We show that the condition holds, for example, when all chance moves are public, that is, both players observe all chance moves. This implies that an optimal EFCE, EFCCE and NFCCE can be computed in polynomial time in the game size in two-player games with public chance moves, providing the biggest positive complexity result surrounding extensive-form correlation in more than a decade.

==> text/relationship_V_Xi.tex <==
\section{New Result about the Relationship Between $\cV$ and $\Xi$}

As already noted by~\citet{Stengel08:Extensive}, the inclusion $\Xi \subseteq \cV$ holds trivially in any game. The reverse inclusion, $\Xi \supseteq \cV$ was shown for two-player games without chance moves, but no complete characterization as to when that reverse inclusion holds is currently known. In \cref{thm:xi equal vonS}, we contribute a new connection between the reverse inclusion $\Xi \supseteq \cV$ and the integrality of the vertices of the \vsfp{} (the proof is in \cref{app:xi equal vonS}.

\begin{restatable}{theorem}{thmvinxi}\label{thm:xi equal vonS}
  Let $\Gamma$ be a two-player perfect-recall extensive-form game, let $\cV$ be its \vsfp{}, and let $\Xi$ be its polytope of correlation plans. Then, $\Xi = \cV$ if and only if all vertices of $\cV$ have integer $\{0,1\}$ coordinates.
\end{restatable}

%\cref{thm:xi equal vonS} connects a continuous, analytical statement (the inclusion of the polytope $\cV$ into the polytope $\Xi$) with a discrete, combinatorial statement about the integrality of the vertices of $\cV$. This will be recurring theme in this paper: the analytical point of view of $\cV$ and the combinatorial aspect of it are tightly interconnected.

In the rest of this paper, we set out to study under what conditions the integrality of the vertices of $\cV$ can be shown. Our proof fundamentally relies on a particular structural decomposition theorem for the \vsfp{}, that we introduce in the next section. 
